Tile Pattern KL-Divergence for Analysing and Evolving Game Levels

This paper provides a detailed investigation of using the Kullback-Leibler (KL) Divergence as a way to compare and analyse game-levels, and hence to use the measure as the objective function of an evolutionary algorithm to evolve new levels. We describe the benefits of its asymmetry for level analysis and demonstrate how (not surprisingly) the quality of the results depends on the features used. Here we use tile-patterns of various sizes as features. When using the measure for evolution-based level generation, we demonstrate that the choice of variation operator is critical in order to provide an efficient search process, and introduce a novel convolutional mutation operator to facilitate this. We compare the results with alternative generators, including evolving in the latent space of generative adversarial networks, and Wave Function Collapse. The results clearly show the proposed method to provide competitive performance, providing reasonable quality results with very fast training and reasonably fast generation.

==> table_backup.tex <==
\begin{table*}[]
\begin{tabular}{lllll}
    Generator & training time avg & training time sd & generation time avg & generation time sd\\
    MarioGAN & 1800 & - & <1 & <1 \\
    KL-DIV 2x2 & & & & \\
    KL-DIV  3x3 & & & & \\
    KL-DIV  4x4 & & & & \\
    KL-DIV  5x14 & & & & \\
    WFC 2x2  & - & - &  16 & 2.245833e-05 \\
    WFC 3x3  & - & - &  336 & 0.0008743991\\
    WFC 4x4 & - & - & 1529 & 0.005801038\\
\end{tabular}
\caption{times (in seconds)}
\end{table*}

\begin{table*}
\begin{tabular}{lllllll}
    Generator & kldiv1 mean & kldiv1 sd & kldiv2 mean & kldiv2 sd & kldiv sym mean & kldiv sym sd\\
    MarioGAN random & 0.075638975 & 0.025861675 & 0.008271824 & 0.008412912 & 0.083910799 & 0.026285863\\
    MarioGAN optimised & 0.06061444 &  0.026928012 & 0.01068297 & 0.009127578 & 0.07129742 & 0.027540680\\
    KL-DIV 2x2 & & & & & &\\
    KL-DIV  3x3 & & & & & &\\
    KL-DIV  4x4 & & & & & &\\
    KL-DIV  5x14 & & & & & &\\
    WFC 2x2  & 0.0572468026 & 0.022571985 & 0.0001487268 & 0.000211757 & 0.0573955294 & 0.022595437\\
    WFC 3x3  & 0.0792393378 & 0.0293499473 & 0.0003634005 & 0.0004592225 & 0.0796027383 & 0.0293814394\\
    WFC 4x4  & 0.0896729215 & 0.0242442385 & 0.0003405128 & 0.0003269759 & 0.0900134343 & 0.0243077412\\
\end{tabular}
\caption{kldiv 2x2 filter from 100 levels}
\end{table*}

\begin{table*}
\begin{tabular}{lllllll}
    Generator & kldiv1 mean & kldiv1 sd & kldiv2 mean & kldiv2 sd & kldiv sym mean & kldiv sym sd\\
    MarioGAN random & 0.15535632 & 0.02923176 & 0.03522657 & 0.02540698 &  0.19058289 & 0.03785990\\
    MarioGAN optimised & 0.14167389 & 0.02793783 & 0.04459437 & 0.02809841 & 0.18626826 & 0.03746278\\
    KL-DIV 2x2 & & & & & &\\
    KL-DIV  3x3 & & & & & &\\
    KL-DIV  4x4 & & & & & &\\
    KL-DIV  5x14 & & & & & &\\
    WFC 2x2  & 0.15028419 & 0.02854969 & 0.03745101 & 0.02413930 & 0.18773520 & 0.03266582\\
    WFC 3x3  & 0.1553896069 & 0.0323769856 & 0.0005850094 & 0.0005250785 & 0.1559746163 & 0.0325614578\\
    WFC 4x4  & 0.1628538258 & 0.029406855 & 0.0005911714 & 0.000452486 & 0.1634449972 & 0.029691015\\
\end{tabular}
\caption{kldiv 3x3 filter from 100 levels}
\end{table*}

\begin{table*}
\begin{tabular}{lllllll}
    Generator & kldiv1 mean & kldiv1 sd & kldiv2 mean & kldiv2 sd & kldiv sym mean & kldiv sym sd\\
    MarioGAN random & 0.26006218 & 0.03443573 & 0.08303578 & 0.05042410 & 0.34309796 & 0.06516000\\
    MarioGAN optimised & 0.2488887 & 0.03613996 & 0.1034942 & 0.05298159 & 0.3523829 & 0.06525710\\
    KL-DIV 2x2 & & & & & &\\
    KL-DIV  3x3 & & & & & &\\
    KL-DIV  4x4 & & & & & &\\
    KL-DIV  5x14 & & & & & &\\
    WFC 2x2  & 0.2627611 & 0.03192529 & 0.1056535 & 0.05849823 & 0.3684146 & 0.06152475\\
    WFC 3x3  & 0.25353618 & 0.03756693 & 0.02053327 & 0.02246265 & 0.27406945 & 0.03985006\\
    WFC 4x4  & 0.255685923 & 0.0347831680 & 0.001067001 & 0.0008873932 & 0.256752924 & 0.0354352237\\
\end{tabular}
\caption{kldiv 4x4 filter from 100 levels}
\end{table*}

